Complex orientations of real algebraic surfaces

We study natural additional structures on real algebraic surfaces with trivial first homology mod 2 of the complexification. If the set of real points realizes the zero of the second homology mod 2 of the complexification, then the set of real points is equipped with a pair of opposite orientations and a Spin structure. If the set of real points realizes the same homology class as the complexification of a real curve on the surface, then the complement of the curve in set of real points is equipped a pair of opposite orientations, which do not extend across the curve, and the whole set of real points is equipped with a Pin^- structure. These constructions are similar to the complex orientations of real algebraic curves dividing their complexifications and generalize to high dimensions.

==> virodef.tex <==
\chardef\tempcat=\the\catcode`\@ \catcode`\@=11
\def\russian{\rus}
\def\p{\partial}
\def\6(#1,#2,#3,#4,#5,#6){\left|\matrix #1&#2&#3\\#4&#5&#6\endmatrix\right|}
\def\conj{\mathop{\roman{conj}}\nolimits}
\def\rnk{\mathop{\roman{rk}}\nolimits}
\def\Tors{\mathop{\roman{Tors}}\nolimits}
\def\Im{\mathop{\roman{Im}}\nolimits}
\def\Rp{\mathop{\roman{Re}}\nolimits}
\def\Ker{\mathop{\roman{Ker}}\nolimits}
\def\tr{\mathop{\roman{tr}}\nolimits}
\def\Coker{\mathop{\roman{Coker}}\nolimits}
\def\Int{\mathop{\roman{Int}}\nolimits}
\def\Cl{\mathop{\roman{Cl}}\nolimits}
\def\Fr{\mathop{\roman{Fr}}\nolimits}
\def\id{\mathop{\roman{id}}\nolimits}
\def\inj{\mathop{\roman{in}}\nolimits}
\def\sign{\mathop{\roman{sign}}\nolimits}
\def\sminus{\smallsetminus}
\def\gap{\phantom{$\sum_{aa_{a_a}}^{a^a}ggggap$}}
\def\rpp{\R P^2}
\def\cpp{\Bbb CP^2}
\def\ca{\Bbb CA}
\def\ra{\R A}
\def\empt{\varnothing}
\def\1{\hbox{\rm\rlap {1}\hskip.03in{\lat I}}}
\def\CC{\Bbb C}
\def\C{\Bbb C}
\def\ZZ{\Bbb Z}
\def\Z{\Bbb Z}
\def\QQ{\Bbb Q}
\def\Q{\Bbb Q}
\def\RR{\Bbb R}
\def\R{\Bbb R}
%\def\R{\hbox{\rm\rlap {\lat I}\hskip.02in{\lat R}}}
\def\NN{\Bbb N}
\def\N{\Bbb N}
\def\Ga{\alpha}
\def\Gb{\beta}
\def\GG{\Gamma}
\def\Gg{\gamma}
\def\Ge{\varepsilon}
\def\GD{\Delta}
\def\Gd{\delta}
\def\Gz{\zeta}
\def\Gth{\theta}
\def\Gi{\iota}
\def\Gk{\varkappa}
\def\Gl{\lambda}
\def\Gr{\rho}
\def\Gs{\sigma}
\def\Gt{\tau}
\def\Gf{\varphi}
\def\GTh{\Theta}
\def\GS{\Sigma}
\def\GL{\Lambda}
\def\Go{\omega}
\def\GO{\Omega}
\def\Gn{\nu}
\newcount\endnotecount@
\endnotecount@\z@
%\long
\def\endnote#1{\global\advance\endnotecount@\@ne
             $(^{\number\endnotecount@})$\enskip
         \expandafter%\long
\gdef\csname endnote\romannumeral\endnotecount@\endcsname
			 {\ifL@tin\lat\else\rus\fi \ignorespaces#1 }}
% \long
\outer\def\makeendnotes{\ifnum\endnotecount@>\z@
			   {\vskip0.5in
	\heading \ifL@tin\lat Notes \else\rus Примечания \fi\endheading
				\count@\z@
				\loop\ifnum\count@<\endnotecount@
                     \advance\count@\@ne
                     $(^{\number\count@})$\enspace
	 \csname endnote\romannumeral\count@\endcsname\vskip\parskip \repeat}\fi}
\def\abz{\vskip\parskip}
\def\n#1{{\bf #1}\hskip.5em\relax}
\def\headfont@{\bf}
\catcode`\@=\tempcat \let\tempcat=\undefined

